Persistent Combinatorial Model of the Restricted Second Configuration Space of Metric Star Graphs

In this work, we present explicit constructions and computations of representative cycles for a nontrivial 2-parameter persistence module arising from the configuration space of metric star graphs. For all edge-length vector $\mathbf{L}=(L_1, L_2, \dots, L_k)\in(\mathbb{R}_{>0})^k$, we construct a bipartite weighted graph $(G_k)_{\mathbf{L}}$ and define filtering functions on the set of vertices and set of edges of $(G_k)_{\mathbf{L}}$ to obtain a filtration (denoted by $(G_k)_{-,\mathbf{L}}$) consisting of geometric realization of subgraphs of $(G_k)_{\mathbf{L}}$. We show that such a filtration is naturally isomorphic to the filtration of the restricted second configuration space of metric star graphs $(\mathsf{Star}_k)^2_{r,\mathbf{L}}$ concerning the restraint parameter $r$ and an (arbitrary but fixed) edge-length vector $\mathbf{L}$. Additionally, we show that the filtration $(G_k)_{-,\mathbf{L}}$ is compatible with the edge-length vector $\mathbf{L}$ up to isotopy, establishing an equivalence between the associated $(k+1)$-parameter persistence modules $PH_{i}((\mathsf{Star}_k)^2_{-,-};\mathbb{F})$ and $PH_{i}((G_k)_{-,-};\mathbb{F})$. We call the (multi-)filtration $(G_k)_{-,-}$ a \textit{persistent combinatorial model} of the multifiltration $(\mathsf{Star}_k)^2_{-,-}$. Using this model, we construct explicit compatible cycle representatives for $PH_{1}((\mathsf{Star}_k)^2_{-,-};\mathbb{F})$ in the bifiltration obtained by fixing $L_2, \dots, L_k > 0$ and varying only $r$ and $L_1$.

==> chapters/k=5.tex <==
\section{The Indecomposable Direct Summands of $PH_1((\mathsf{Star}_5)^2_{-,-};\mathbb{F})$}
Now we compute the indecomposable direct summands for $PH_1((\mathsf{Star}_5)^2_{-,-};\mathbb{F})$, where ${\mathbf{L}}=(L,L_2,L_3,L_4,L_5)$ with arbitrary but fixed $L_2,L_3,L_4,L_5\in\mathbb{R}_{>0}$. Without loss of generality, we assume $L_2\leq L_3\leq L_4\leq L_5$. We need to find a basis for $PH_1((\mathsf{Star}_5)^2_{r,{\mathbf{L}}};\mathbb{F})$ such that the basis elements are compatible when $(r,L)\leq (r',L')$. The rank of $H_1((\mathsf{Star}_5)^2_{r,\mathbf{L}})$ for all $(r,L)$ follows directly from Theorem~\ref{thm:4:3}, Theorem~\ref{cor:4.4}, and Theorem~\ref{thm:4.5}. See Figure~\ref{fig:20}.

\begin{figure}[htbp!]
    \centering
\resizebox{0.5\textwidth}{!}{


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp6998877377278565] 
\draw  [draw opacity=0][fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.4 ] (126,24) -- (247.5,24) -- (247.5,223) -- (126,223) -- cycle ;
%Straight Lines [id:da5197325224885494] 
\draw    (2,223) -- (283.5,223) ;
\draw [shift={(285.5,223)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da28337336688824444] 
\draw    (22,243) -- (22,16) ;
\draw [shift={(22,14)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da44697088386633643] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (21.5,223) -- (219.5,25) ;
%Straight Lines [id:da061384162782543994] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (60.5,223) -- (246.5,37) ;
%Straight Lines [id:da7780784304773196] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (60.5,223) -- (60.5,24) ;
%Straight Lines [id:da7757796652676971] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (126,223) -- (126,175) -- (126,24) ;
%Straight Lines [id:da5571649594188037] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (94,223) -- (94,24) ;
%Straight Lines [id:da7215393415997637] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (94,223) -- (248,69) ;
%Straight Lines [id:da4663748241180692] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (126,223) -- (247.5,101.5) ;
%Straight Lines [id:da06991346789858599] 
\draw [color={rgb, 255:red, 45; green, 139; blue, 42 }  ,draw opacity=1 ][line width=0.75]    (203,223) -- (203,24) ;
%Straight Lines [id:da4969156379573655] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (159,223) -- (159,107) -- (159,24) ;
%Straight Lines [id:da8544007529858177] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (159,223) -- (247,135) ;
%Shape: Polygon [id:ds5452302117770466] 
\draw  [draw opacity=0][fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.4 ] (93.5,152) -- (126.5,118) -- (126,223) -- (94,223) -- cycle ;

% Text Node
\draw (5,5.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$L$};
% Text Node
\draw (287.5,226.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$r$};
% Text Node
\draw (49,227.4) node [anchor=north west][inner sep=0.75pt]    {$L_{2}$};
% Text Node
\draw (85,227.4) node [anchor=north west][inner sep=0.75pt]    {$L_{3}$};
% Text Node
\draw (119,227.4) node [anchor=north west][inner sep=0.75pt]    {$L_{4}$};
% Text Node
\draw (181,228.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,opacity=1 ]  {$L_{2} +L_{3}$};
% Text Node
\draw (150.75,227.4) node [anchor=north west][inner sep=0.75pt]    {$L_{5}$};
% Text Node
\draw (72,95.4) node [anchor=north west][inner sep=0.75pt]    {$5$};
% Text Node
\draw (42,203.4) node [anchor=north west][inner sep=0.75pt]    {$5$};
% Text Node
\draw (33,95.4) node [anchor=north west][inner sep=0.75pt]    {$11$};
% Text Node
\draw (104,95.4) node [anchor=north west][inner sep=0.75pt]    {$1$};
% Text Node
\draw (72,179.4) node [anchor=north west][inner sep=0.75pt]    {$1$};
% Text Node
\draw (80,203.4) node [anchor=north west][inner sep=0.75pt]    {$1$};


\end{tikzpicture}
}
    \caption{The rank of $H_1((\mathsf{Star}_5)^2_{r,\mathbf{L}})$ for all $(r,L)$ in the shaded region. In particular, $\rank H_1((\mathsf{Star}_k)^2_{r,\mathbf{L}})=0$ when $(r,L)$ lies in the gray region.}
    \label{fig:20}
\end{figure}


Applying Theorem~\ref{thm-sim-1'}, we construct the poset of chambers (denoted by $(P,\leq)$) and the representation $M$ over $(P,\leq)$ as follows:

\begin{figure}[htbp!]
    \centering
    % First subfigure
    \begin{subfigure}{0.45\textwidth}
        \centering
        \begin{tikzcd}
\bullet & \bullet \arrow[l] & \bullet \arrow[l]\\
\bullet \arrow[u] & \bullet\arrow[u] \arrow[l] & \\
 & \bullet\arrow[u] & 
\end{tikzcd}
        \caption{The Hasse Diagram of the Poset of Chambers}
        \label{fig:Poset_P}
    \end{subfigure}
    \hfill
    % Second subfigure
    \begin{subfigure}{0.45\textwidth}
        \centering
                \begin{tikzcd}
\mathbb{F}^{11} & \mathbb{F}^{5} \arrow[l] & \mathbb{F} \arrow[l]\\
\mathbb{F}^{5} \arrow[u] & \mathbb{F}\arrow[u] \arrow[l] & \\
 & \mathbb{F}\arrow[u] & 
\end{tikzcd}
        \caption{Poset Representation $M$}
        \label{fig:Rep/P}
    \end{subfigure}
    
    \caption{}
\end{figure}

Notice that $(G_5)_{r,L}$ is at most a 1-dimensional CW complex, i.e., a (geometric) graph, and the set consists of its fundamental cycles forms a basis for $H_1((G_5)_{r,L};\mathbb{F})$. Similar to the case when $k=4$, we smooth all vertices of $(G_5)_{\mathbf{L}}$ of degree 2 and call the resulting graph the reduced $(G_5)_{\mathbf{L}}$.

When $r<L$ and $r<L_2$, the fundamental cycles of the reduced $(G_5)_{\mathbf{L}}$ are provided in Figure~\ref{fig:fundamental_cycles_G5}.

\begin{figure}[htbp!]
    \centering
    % first figure
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{chapters/k=5, indecomposable summands/cycle_1.png}
        \caption{$X_1$}
    \end{subfigure}
    \hfill
    % second figure
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{chapters/k=5, indecomposable summands/cycle_2.png}
        \caption{$X_2$}
    \end{subfigure}
    \hfill
    % third figure
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{chapters/k=5, indecomposable summands/cycle_3.png}
        \caption{$X_3$}
    \end{subfigure}

    % fourth figure
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{chapters/k=5, indecomposable summands/cycle_4.png}
        \caption{$X_4$}
    \end{subfigure}
    \hfill
    % fifth figure
    \begin{subfigure}{0.3\textwidth}
        \centering
        
    \includegraphics[width=\linewidth]{chapters/k=5, indecomposable summands/cycle_5.png}
        \caption{$X_5$}
    \end{subfigure}
    \hfill
    % sixth figure
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{chapters/k=5, indecomposable summands/cycle_6.png}
        \caption{$X_6$}
    \end{subfigure}

    % seventh figure
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{chapters/k=5, indecomposable summands/cycle_7.png}
        \caption{$X_7$}
    \end{subfigure}
    \hfill
    % eighth figure
    \begin{subfigure}{0.3\textwidth}
        \centering
        
    \includegraphics[width=\linewidth]{chapters/k=5, indecomposable summands/cycle_8.png}
        \caption{$X_8$}
    \end{subfigure}
    \hfill
    % ninth figure
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{chapters/k=5, indecomposable summands/cycle_9.png}
        \caption{$X_9$}
    \end{subfigure}
    
     % tenth figure
    \begin{subfigure}{0.3\textwidth}
        \centering
        
    \includegraphics[width=\linewidth]{chapters/k=5, indecomposable summands/cycle_10.png}
        \caption{$X_{10}$}
    \end{subfigure}
    % ninth figure
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{chapters/k=5, indecomposable summands/cycle_11.png}
        \caption{$X_{11}$}
    \end{subfigure}
    \hfill
    \caption{Generators of $H_1(\lVert (G_5)_{r,\mathbf{L}}\rVert)$} when $r$ is small.
    \label{fig:fundamental_cycles_G5}
\end{figure}

With respect to the fundamental cycles, the representation $M$ can be written as:
\begin{center}
\begin{tikzcd}[%
    >=stealth,
    node distance=3cm,
    on grid,
    auto
  ]
  \parbox[c]{6.3cm}{%
    $\langle X_1, X_2, X_3, X_4, X_5, X_6, X_7, X_8, X_9, X_{10}, X_{11} \rangle$%
  } 
  & \langle X_2, X_3, X_7, X_8, X_{11}\rangle \arrow[l, hook] 
  & \langle X_3\rangle \arrow[l, hook] \\
  \langle X_4\Delta X_{11}, X_5\Delta X_{10}, X_7\Delta X_{10}, X_9\Delta X_{10}, X_{10}\Delta X_{11} \rangle \arrow[u]
  & \langle X_7\Delta X_{11}\rangle \arrow[u] \arrow[l]
  &
\end{tikzcd}
\end{center}

Note that every linear transformation in the representation $M$ is injective since $(G_5)_{\mathbf{L}}$ is at most 1-dimensional. In particular, the linear transformations in the top row are inclusions. A compatible basis for the vector spaces in the representation $M$ is given below.
\begin{center}
\begin{tikzcd}[%
    >=stealth,
    node distance=3cm,
    on grid,
    auto
  ]
  \parbox[c]{6.3cm}{%
    $\langle X_1, X_2, X_3, X_6, X_8, X_{11}, X_4\Delta X_{11}, X_5\Delta X_{10},$\\
    $X_7\Delta X_{11}, X_9\Delta X_{10}, X_{10}\Delta X_{11} \rangle$%
  } 
  & \langle X_2, X_3, X_8, X_{11}, X_7\Delta X_{11}\rangle \arrow[l, hook] 
  & \langle X_3\rangle \arrow[l, hook] \\
  \langle X_4\Delta X_{11}, X_5\Delta X_{10}, X_7\Delta X_{11}, X_9\Delta X_{10}, X_{10}\Delta X_{11} \rangle \arrow[u, hook]
  & \langle X_7\Delta X_{11}\rangle \arrow[u, hook] \arrow[l, hook]
  &
\end{tikzcd}
\end{center}

Hence $M$ is interval-decomposable, and its indecomposable direct summands are

\begin{figure}[htbp!]
    \centering
    % First subfigure
    \begin{subfigure}{0.4\textwidth}
        \centering
        \begin{tikzcd}
    \langle X_7\Delta X_{11}\rangle 
  & \langle  X_7\Delta X_{11}\rangle \arrow[l, hook] 
  & 0 \arrow[l, hook] \\
  \langle X_7\Delta X_{11}\rangle \arrow[u, hook]
  & \langle X_7\Delta X_{11}\rangle \arrow[u, hook] \arrow[l, hook]
  &\\
  & \langle X_7\Delta X_{11}\rangle \arrow[u, hook]
  &
\end{tikzcd}
        \caption{}
    \end{subfigure}%
    \hfill
    % Second subfigure
    \begin{subfigure}{0.3\textwidth}
        \centering
        \begin{tikzcd}
    \langle X_3\rangle 
  & \langle  X_3\rangle \arrow[l, hook] 
  & X_3 \arrow[l, hook] \\
  0 \arrow[u, hook]
  &0 \arrow[u, hook] \arrow[l, hook]
  &\\
  & 0 \arrow[u, hook]
  &
\end{tikzcd}
        \caption{}
    \end{subfigure}%
    \hfill
    % Third subfigure
    \begin{subfigure}{0.3\textwidth}
        \centering
        \begin{tikzcd}
    \langle X_i\rangle 
  & \langle  X_i\rangle \arrow[l, hook] 
  & 0 \arrow[l, hook] \\
  0 \arrow[u, hook]
  &0 \arrow[u, hook] \arrow[l, hook]
  &\\
  & 0 \arrow[u, hook]
  &
\end{tikzcd}
        \caption{For $i=2,8,11$}
    \end{subfigure}
    % Fourth subfigure
    \begin{subfigure}{0.3\textwidth}
        \centering
        \begin{tikzcd}
    \langle X_i\rangle 
  & 0\arrow[l, hook] 
  & 0 \arrow[l, hook] \\
  0 \arrow[u, hook]
  &0 \arrow[u, hook] \arrow[l, hook]
  &\\
  & 0 \arrow[u, hook]
  &
\end{tikzcd}
        \caption{For $i=1,6$}
    \end{subfigure}%
    % Fifth subfigure
    \begin{subfigure}{0.3\textwidth}
        \centering
        \begin{tikzcd}
    \langle X_i\Delta X_{10}\rangle 
  & 0\arrow[l, hook] 
  & 0 \arrow[l, hook] \\
  \langle X_i\Delta X_{10}\rangle  \arrow[u, hook]
  &0 \arrow[u, hook] \arrow[l, hook]
  &\\
  & 0 \arrow[u, hook]
  &
\end{tikzcd}
        \caption{For $i=5,9$}
    \end{subfigure}%
    % Sixth subfigure
    \begin{subfigure}{0.3\textwidth}
        \centering
        \begin{tikzcd}
    \langle X_i\Delta X_{11}\rangle 
  & 0\arrow[l, hook] 
  & 0 \arrow[l, hook] \\
  \langle X_i\Delta X_{11}\rangle  \arrow[u, hook]
  &0 \arrow[u, hook] \arrow[l, hook]
  &\\
  & 0 \arrow[u, hook]
  &
\end{tikzcd}
        \caption{For $i=4,10$}
    \end{subfigure}%
    \caption{}
    \label{fig:inde_summands_G5}
\end{figure}

\begin{theorem}\label{thm:5.9}
    Let $\mathbf{L}=(L,L_2,L_3,L_4,L_5)$ where $L_2\leq L_3\leq L_4 \leq L_5$ are fixed positive real numbers. The indecomposable direct summands of $PH_1((\mathsf{Star}_5)^2_{-,-};\mathbb{F})$ are the interval modules whose supports are given by the shaded regions in Figure~\ref{fig:G5_summands}.
    \begin{figure}[htbp!]
    \centering
     \begin{minipage}{0.333\textwidth}
            \centering
            \resizebox{\textwidth}{!}{
            

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da5197325224885494] 
\draw    (2,223) -- (283.5,223) ;
\draw [shift={(285.5,223)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da28337336688824444] 
\draw    (22,243) -- (22,16) ;
\draw [shift={(22,14)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da44697088386633643] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (21.5,223) -- (219.5,25) ;
%Straight Lines [id:da061384162782543994] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (60.5,223) -- (246.5,37) ;
%Straight Lines [id:da7780784304773196] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (60.5,223) -- (60.5,24) ;
%Straight Lines [id:da7757796652676971] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (126,223) -- (126,175) -- (126,24) ;
%Straight Lines [id:da5571649594188037] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (94,223) -- (94,24) ;
%Straight Lines [id:da7215393415997637] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (94,223) -- (248,69) ;
%Straight Lines [id:da4663748241180692] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (126,223) -- (247.5,101.5) ;
%Straight Lines [id:da06991346789858599] 
\draw [color={rgb, 255:red, 45; green, 139; blue, 42 }  ,draw opacity=1 ][line width=0.75]    (203,223) -- (203,24) ;
%Straight Lines [id:da4969156379573655] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (159,223) -- (159,107) -- (159,24) ;
%Straight Lines [id:da8544007529858177] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (159,223) -- (247,135) ;
%Shape: Rectangle [id:dp02186288617861043] 
\draw  [draw opacity=0][fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=0.4 ] (21.5,24) -- (94,24) -- (94,223) -- (21.5,223) -- cycle ;

% Text Node
\draw (5,5.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$L$};
% Text Node
\draw (287.5,226.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$r$};
% Text Node
\draw (49,227.4) node [anchor=north west][inner sep=0.75pt]    {$L_{2}$};
% Text Node
\draw (85,227.4) node [anchor=north west][inner sep=0.75pt]    {$L_{3}$};
% Text Node
\draw (119,227.4) node [anchor=north west][inner sep=0.75pt]    {$L_{4}$};
% Text Node
\draw (181,228.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,opacity=1 ]  {$L_{2} +L_{3}$};
% Text Node
\draw (150.75,227.4) node [anchor=north west][inner sep=0.75pt]    {$L_{5}$};


\end{tikzpicture}
    }
            \subcaption{Multiplicity = 1}
            \label{fig:sub-a}
        \end{minipage}%
     \begin{minipage}{0.333\textwidth}
            \centering
            \resizebox{\textwidth}{!}{
            

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da5197325224885494] 
\draw    (2,223) -- (283.5,223) ;
\draw [shift={(285.5,223)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da28337336688824444] 
\draw    (22,243) -- (22,16) ;
\draw [shift={(22,14)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da44697088386633643] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (21.5,223) -- (219.5,25) ;
%Straight Lines [id:da061384162782543994] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (60.5,223) -- (246.5,37) ;
%Straight Lines [id:da7780784304773196] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (60.5,223) -- (60.5,24) ;
%Straight Lines [id:da7757796652676971] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (126,223) -- (126,175) -- (126,24) ;
%Straight Lines [id:da5571649594188037] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (94,223) -- (94,24) ;
%Straight Lines [id:da7215393415997637] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (94,223) -- (248,69) ;
%Straight Lines [id:da4663748241180692] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (126,223) -- (247.5,101.5) ;
%Straight Lines [id:da06991346789858599] 
\draw [color={rgb, 255:red, 45; green, 139; blue, 42 }  ,draw opacity=1 ][line width=0.75]    (203,223) -- (203,24) ;
%Straight Lines [id:da4969156379573655] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (159,223) -- (159,107) -- (159,24) ;
%Straight Lines [id:da8544007529858177] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (159,223) -- (247,135) ;
%Shape: Polygon [id:ds8403320034065876] 
\draw  [draw opacity=0][fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.4 ] (126,24) -- (126.5,119) -- (21.5,223) -- (22.5,23) -- cycle ;

% Text Node
\draw (5,5.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$L$};
% Text Node
\draw (287.5,226.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$r$};
% Text Node
\draw (49,227.4) node [anchor=north west][inner sep=0.75pt]    {$L_{2}$};
% Text Node
\draw (85,227.4) node [anchor=north west][inner sep=0.75pt]    {$L_{3}$};
% Text Node
\draw (119,227.4) node [anchor=north west][inner sep=0.75pt]    {$L_{4}$};
% Text Node
\draw (181,228.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,opacity=1 ]  {$L_{2} +L_{3}$};
% Text Node
\draw (150.75,227.4) node [anchor=north west][inner sep=0.75pt]    {$L_{5}$};


\end{tikzpicture}
    }
            \subcaption{Multiplicity = 1}
            \label{fig:sub-b}
        \end{minipage}%
    \begin{minipage}{0.333\textwidth}
            \centering
            \resizebox{\textwidth}{!}{
            

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da5197325224885494] 
\draw    (2,223) -- (283.5,223) ;
\draw [shift={(285.5,223)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da28337336688824444] 
\draw    (22,243) -- (22,16) ;
\draw [shift={(22,14)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da44697088386633643] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (21.5,223) -- (219.5,25) ;
%Straight Lines [id:da061384162782543994] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (60.5,223) -- (246.5,37) ;
%Straight Lines [id:da7780784304773196] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (60.5,223) -- (60.5,24) ;
%Straight Lines [id:da7757796652676971] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (126,223) -- (126,175) -- (126,24) ;
%Straight Lines [id:da5571649594188037] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (94,223) -- (94,24) ;
%Straight Lines [id:da7215393415997637] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (94,223) -- (248,69) ;
%Straight Lines [id:da4663748241180692] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (126,223) -- (247.5,101.5) ;
%Straight Lines [id:da06991346789858599] 
\draw [color={rgb, 255:red, 45; green, 139; blue, 42 }  ,draw opacity=1 ][line width=0.75]    (203,223) -- (203,24) ;
%Straight Lines [id:da4969156379573655] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (159,223) -- (159,107) -- (159,24) ;
%Straight Lines [id:da8544007529858177] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (159,223) -- (247,135) ;
%Shape: Polygon [id:ds6720163127685481] 
\draw  [draw opacity=0][fill={rgb, 255:red, 189; green, 16; blue, 224 }  ,fill opacity=0.4 ] (94,24) -- (93.5,152) -- (21.5,223) -- (21.5,23) -- cycle ;

% Text Node
\draw (5,5.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$L$};
% Text Node
\draw (287.5,226.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$r$};
% Text Node
\draw (49,227.4) node [anchor=north west][inner sep=0.75pt]    {$L_{2}$};
% Text Node
\draw (85,227.4) node [anchor=north west][inner sep=0.75pt]    {$L_{3}$};
% Text Node
\draw (119,227.4) node [anchor=north west][inner sep=0.75pt]    {$L_{4}$};
% Text Node
\draw (181,228.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,opacity=1 ]  {$L_{2} +L_{3}$};
% Text Node
\draw (150.75,227.4) node [anchor=north west][inner sep=0.75pt]    {$L_{5}$};


\end{tikzpicture}
    }
            \subcaption{Multiplicity = 3}
            \label{fig:sub-c}
        \end{minipage}
     \begin{minipage}{0.333\textwidth}
            \centering
            \resizebox{\textwidth}{!}{
            

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da5197325224885494] 
\draw    (2,223) -- (283.5,223) ;
\draw [shift={(285.5,223)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da28337336688824444] 
\draw    (22,243) -- (22,16) ;
\draw [shift={(22,14)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da44697088386633643] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (21.5,223) -- (219.5,25) ;
%Straight Lines [id:da061384162782543994] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (60.5,223) -- (246.5,37) ;
%Straight Lines [id:da7780784304773196] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (60.5,223) -- (60.5,24) ;
%Straight Lines [id:da7757796652676971] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (126,223) -- (126,175) -- (126,24) ;
%Straight Lines [id:da5571649594188037] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (94,223) -- (94,24) ;
%Straight Lines [id:da7215393415997637] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (94,223) -- (248,69) ;
%Straight Lines [id:da4663748241180692] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (126,223) -- (247.5,101.5) ;
%Straight Lines [id:da06991346789858599] 
\draw [color={rgb, 255:red, 45; green, 139; blue, 42 }  ,draw opacity=1 ][line width=0.75]    (203,223) -- (203,24) ;
%Straight Lines [id:da4969156379573655] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (159,223) -- (159,107) -- (159,24) ;
%Straight Lines [id:da8544007529858177] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (159,223) -- (247,135) ;
%Shape: Polygon [id:ds943166919753873] 
\draw  [draw opacity=0][fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=0.4 ] (60.5,24) -- (59.5,185) -- (21.5,223) -- (21.5,24) -- cycle ;

% Text Node
\draw (5,5.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$L$};
% Text Node
\draw (287.5,226.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$r$};
% Text Node
\draw (49,227.4) node [anchor=north west][inner sep=0.75pt]    {$L_{2}$};
% Text Node
\draw (85,227.4) node [anchor=north west][inner sep=0.75pt]    {$L_{3}$};
% Text Node
\draw (119,227.4) node [anchor=north west][inner sep=0.75pt]    {$L_{4}$};
% Text Node
\draw (181,228.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,opacity=1 ]  {$L_{2} +L_{3}$};
% Text Node
\draw (150.75,227.4) node [anchor=north west][inner sep=0.75pt]    {$L_{5}$};


\end{tikzpicture}
    }
            \subcaption{Multiplicity = 2}
            \label{fig:sub-d}
        \end{minipage}%  
     \begin{minipage}{0.333\textwidth}
            \centering
            \resizebox{\textwidth}{!}{
            

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da5197325224885494] 
\draw    (2,223) -- (283.5,223) ;
\draw [shift={(285.5,223)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da28337336688824444] 
\draw    (22,243) -- (22,16) ;
\draw [shift={(22,14)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da44697088386633643] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (21.5,223) -- (219.5,25) ;
%Straight Lines [id:da061384162782543994] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (60.5,223) -- (246.5,37) ;
%Straight Lines [id:da7780784304773196] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (60.5,223) -- (60.5,24) ;
%Straight Lines [id:da7757796652676971] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (126,223) -- (126,175) -- (126,24) ;
%Straight Lines [id:da5571649594188037] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (94,223) -- (94,24) ;
%Straight Lines [id:da7215393415997637] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (94,223) -- (248,69) ;
%Straight Lines [id:da4663748241180692] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (126,223) -- (247.5,101.5) ;
%Straight Lines [id:da06991346789858599] 
\draw [color={rgb, 255:red, 45; green, 139; blue, 42 }  ,draw opacity=1 ][line width=0.75]    (203,223) -- (203,24) ;
%Straight Lines [id:da4969156379573655] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (159,223) -- (159,107) -- (159,24) ;
%Straight Lines [id:da8544007529858177] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][line width=0.75]    (159,223) -- (247,135) ;
%Shape: Rectangle [id:dp02186288617861043] 
\draw  [draw opacity=0][fill={rgb, 255:red, 2; green, 18; blue, 208 }  ,fill opacity=0.4 ] (21.5,24) -- (60.5,24) -- (60.5,223) -- (21.5,223) -- cycle ;

% Text Node
\draw (5,5.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$L$};
% Text Node
\draw (287.5,226.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$r$};
% Text Node
\draw (49,227.4) node [anchor=north west][inner sep=0.75pt]    {$L_{2}$};
% Text Node
\draw (85,227.4) node [anchor=north west][inner sep=0.75pt]    {$L_{3}$};
% Text Node
\draw (119,227.4) node [anchor=north west][inner sep=0.75pt]    {$L_{4}$};
% Text Node
\draw (181,228.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,opacity=1 ]  {$L_{2} +L_{3}$};
% Text Node
\draw (150.75,227.4) node [anchor=north west][inner sep=0.75pt]    {$L_{5}$};


\end{tikzpicture}
    }
            \subcaption{Multiplicity = 4}
            \label{fig:sub-e}
        \end{minipage}%  
    \caption{The indecomposable direct summands of $PH_1((\mathsf{Star}_5)^2_{-,-};\mathbb{F})$}
    \label{fig:G5_summands}
    \end{figure}
\end{theorem}



%\begin{corollary}
%$PH_1((\mathsf{Star}_5)^2_{-,-};\mathbb{F})$ is interval-indecomposable.
%\end{corollary}
%\begin{proof}
    %For all $\mathbf{L}=(L,L_2, L_3, L_4, L_5)$, without loss of generality, we may assume $L_2\leq L_3\leq L_4\leq L_5$. $(\mathsf{Star}_5)^2_{r,\mathbf{L}}$ has the following critical hyperplanes in the parameter space:
    %\begin{equation*}
        %\begin{aligned}
            %r&=L\\
            %r&=L_i, \quad\mbox{for all } i=2,3,4,5\\
            %r&=L+L_i, \quad \mbox{for all } i=1,2,3,4,5\\
            %r&=L_i+L_j, \quad \mbox{for all } i,j=2,3,4,5 \mbox{ and } i\neq j
        %\end{aligned}
    %\end{equation*}
%\end{proof}

==> mbboard.tex <==
% blackboard typefaces by Anthony Phan.
% file: mbboard.tex (\TeX' file for mbb's fonts)
% last modification: November 1st, 1999.
%
\catcode`@=11
%
% proofing?
%
\ifx\proofmode\undefined
	\def\symbol@message#1{\relax}%
	\def\symbol@mark#1#2{\relax}%
\else
	\def\symbol@message#1{\medbreak{\noindent\bf #1}
		\medskip\noindent\ignorespaces}%
	\def\symbolsp@cing#1{(\ifcase\number#1 ord\or op%
		\or bin\or rel\or open\or close\or punct%
		\or var\else ???\fi)}%
	\def\symbol@mark#1#2{$#1$ {\tt\string#1}
		\symbolsp@cing{#2},\ \ignorespaces}%
\fi
%
% Symbols declarations: \LaTeX-like commands
%
\def\hexnumber@#1{\ifcase\number#1 0\or 1\or 2\or 3\or 4%
	\or 5\or 6\or 7\or 8\or 9\or A\or B\or C\or D\or E\or F\fi}%
%
\def\DeclareMathSymbol#1#2#3#4{%
	\count255=#2\multiply\count255 by 16
	\advance\count255 by \csname#3fam\endcsname
	\multiply\count255 by 256\advance\count255 by #4
	\ifcat\noexpand#1\relax\mathchardef#1=\count255
	\else\expandafter
		\mathcode\expandafter`\csname#1\endcsname=\count255
	\fi\symbol@mark{#1}{#2}}
%
\def\gobble@quotes#1{\ifx#1"\else#1\fi}
%
\def\@DeclareMathDelimiter#1#2#3#4#5#6{%
	\edef#1{\noexpand\delimiter\noexpand"\gobble@quotes#2%
	\expandafter\hexnumber@\csname#3fam\endcsname\gobble@quotes#4%
	\expandafter\hexnumber@\csname#5fam\endcsname\gobble@quotes#6 }%
	\symbol@mark{#1}{#2}}
%
\def\@xDeclareMathDelimiter#1#2#3#4#5{%
	\count255=\csname#2fam\endcsname
	\multiply\count255 by 256\advance\count255 by #3
	\multiply\count255 by 16
	\advance\count255 by \csname#4fam\endcsname
	\multiply\count255 by 256\advance\count255 by #5
	\expandafter\delcode\expandafter`\csname#1\endcsname=\count255
	\symbol@mark{#1}{#2}}
%
\def\DeclareMathDelimiter#1{%
	\ifcat\noexpand#1\relax
	\def\Large@stuff{\noexpand\delimiter}%
	\expandafter\@DeclareMathDelimiter
	\else\expandafter\@xDeclareMathDelimiter\fi#1}
%
\def\DeclareMathRadical#1#2#3#4#5{%
	\edef#1{\noexpand\radical\noexpand"%
	\expandafter\hexnumber@\csname#2fam\endcsname\gobble@quotes#3%
	\expandafter\hexnumber@\csname#4fam\endcsname\gobble@quotes#5 }%
	\symbol@mark{#1.}{8}}
%
\def\DeclareMathAccent#1#2#3#4{%
        \edef#1{\noexpand\mathaccent\noexpand"%
	\expandafter\hexnumber@\csname#3fam\endcsname\gobble@quotes#4 }%
	\symbol@mark{#1.}{8}}
%
% loading blackboard fonts
%
\font\twelvembb=mbb12 \font\tenmbb=mbb10
\font\ninembb=mbb9    \font\eightmbb=mbb8
\font\sevenmbb=mbb7   \font\sixmbb=mbb6
\font\fivembb=mbb5
%
\skewchar\tenmbb="7F   \skewchar\ninembb="7F \skewchar\eightmbb="7F 
\skewchar\sevenmbb="7F \skewchar\sixmbb="7F  \skewchar\fivembb="7F 
\hyphenchar\tenmbb="2D   \hyphenchar\ninembb="2D \hyphenchar\eightmbb="2D 
\hyphenchar\sevenmbb="2D \hyphenchar\sixmbb="2D  \hyphenchar\fivembb="2D 
%
\newfam\mbbfam
%
% Initialization
% (make changes in your own file if you want different sizes)
%
\textfont\mbbfam=\tenmbb  \scriptfont\mbbfam=\sevenmbb
\scriptscriptfont\mbbfam=\fivembb  \def\mbb{\fam\mbbfam\tenmbb}
\def\mathbb#1{{\fam\mbbfam#1}}
%
\input mbboard.dcl
%
\catcode`@=12
\let\proofmode=\undefined
\endinput




